History-Register Automata

Programs with dynamic allocation are able to create and use an unbounded number of fresh resources, such as references, objects, files, etc. We propose History-Register Automata (HRA), a new automata-theoretic formalism for modelling such programs. HRAs extend the expressiveness of previous approaches and bring us to the limits of decidability for reachability checks. The distinctive feature of our machines is their use of unbounded memory sets (histories) where input symbols can be selectively stored and compared with symbols to follow. In addition, stored symbols can be consumed or deleted by reset. We show that the combination of consumption and reset capabilities renders the automata powerful enough to imitate counter machines, and yields closure under all regular operations apart from complementation. We moreover examine weaker notions of HRAs which strike different balances between expressiveness and effectiveness.

==> closure.tex <==
\section{Closure properties}\label{sec:closure}


History-register automata enjoy good closure properties with respect to regular language operations. In particular, they are closed under union, intersection, concatenation and Kleene star, but not closed under complementation. 

In fact, the design of HRAs is such that the automata for union and intersection come almost for free through a straightforward product construction which is essentially an ordinary product for finite-state automata, modulo reindexing of places to account for duplicate labels (cf.~\cite{RA1}).
%
\cutout{We do not show these constructions formally (they are very similar to those in~\cite{RA1}), but we demonstrate the second one through an example.

\begin{example}
Break $\LL_2$ into two languages.
\end{example}}%
%
The constructions for Kleene star and concatenation are slightly more involved as there is need for passing through intermediate automata which do not touch their initial names. 

We shall need the following technical gadget. Given an $(m,n)$-HRA $\AA$ and a sequence $w$ of $k$ distinct names, we construct a bisimilar $(m,n{+}k)$-HRA, denoted $\fix{\AA}{w}$, in which the names of $w$ appear exclusively in the additional $k$ registers, which, moreover, remain unchanged during computation. The construction will allow us, for instance, to create feedback loops in automata ensuring that after each feedback transition the same initial configuration occurs.
%\rg{TODO: say here that we can use also histories}

\begin{lemma}\label{lem:forclos}
Let $\AA$ be an $(m,n)$-HRA with initial assignment $H_0$ and $w=a_1\ldots a_k$ a sequence of distinct names. We can effectively construct an $(m,n{+}k)$-HRA $\fix{\AA}{w}$ with initial assignment $H_0'$ such that $\fix{\AA}{w}\sim \AA$ and:
\begin{itemize}
\item $H_0'(m{+}n{+}i)=a_i$ for all $i\in[k]$, and $H_0'(i)=H_0(i)\setminus\{a_1,\ldots,a_k\}$ for all $i\in[m{+}n]$;
\item for all reachable configurations $(q,H)$ of $\fix{\AA}{w}$ and all $i>m{+}n$, $H(i)=H_0'(i)$.
\end{itemize}
\end{lemma}

\begin{proof}
We construct $\fix{\AA}{w}=\langle Q',q_0',H_0',\delta',F'\rangle$ as follows. First, we insert/move all names of $w$ to the new registers (places $[m{+}n{+}1,m{+}n{+}k]$), i.e.~we set $H_0'(i)=H_0(i)\setminus\{a_1\ldots a_k\}$ for all $i\in[m{+}n]$, and  $H_0'(m{+}n{+}i)=\{a_i\}$ for each $i\in[k]$. 
The role of the new registers is to constantly store the names in $w$ and act on the behalf of other places when the latter intend to use  those names: during computation, whenever an $a_i$ is captured by a transition of the initial automaton $\AA$, in $\fix{\AA}{w}$ it will be instead simulated by a transition involving the new registers. In order for the simulation to be accurate, we shall inject inside states information specifying the \emph{intended} location of the $a_i$s in the places of $\AA$.
Thus, the states of the new automaton are pairs $(q,f)$, where $q\in Q$ and $f$ is a function recording, for each of the new registers, where would the name of the register appear in the original automaton $\AA$. That is,
\[
Q'=Q\times\{f:[k]\to\PP([m{+}n])\ |\ \forall j\not=j'\!.\, f(j)\cap f(j')\subseteq[m]\}
\] 
while $q_0'=(q_0,\{(i,\{j\ |\ a_i\in H_0(j)\})\ |\ i\in[k]\})$
and $F'=\{(q,f)\in Q'\ |\ q\in F\}$. Finally, $\delta'$ operates just like $\delta$ albeit taking into account the $f$'s of states to figure out the intended positions of the $a_i$s and, at the same time, update the $f$'s after each transition. We therefore include in $\delta'$ precisely the following transitions. Below we write $i^\circ$ for $m{+}n{+}i$.
For each $(q,f)\in Q'$ and $q\trdelta{X,X'}q'\in\delta$,%
\begin{itemize}
\item add a transition $(q,f)\trdelta{X,X'}(q',f)$;
\item if $f(i)=X$ for some $i$ then add $(q,f)\xtrdelta{\{i^\circ\},\{i^\circ\}}(q',f')$ where $f'=f[i\mapsto X']$;
\end{itemize}
Moreover, for each $q\trdelta{X}q'\in\delta$ include $(q,f)\trdelta{X}(q',f')$ where $f'=\{(j,f(j)\setminus X)\ |\ j\in[k]\}$.
\\
Following the above line of reasoning, we can show that  the relation
\[
\{ ((q,H),(q,f,H'))\ |\ \forall i\!\in\![m{+}n].\,H(i)=H'(i)\cup\{a_j\,|\,i\in f(j)\}\}
\]
with $(q,H),(q,f,H')$ reachable configurations, is a bisimulation.
\end{proof}


%We now show that languages recognised by HRAs are closed under union, intersection, concatenation and Kleene star.

We write $\LL\circ\LL'$ for concatenation of languages,
  and $\LL^*$ for Kleene closure of a language.
We use the same definitions as the standard ones for languages over finite alphabets:
  $\LL \circ \LL'$ is $\{\,ww'\mid w\in\LL \,\land\, w'\in \LL'\,\}$,
  and $\LL^*$ is the least fixed-point of the
    equations $\epsilon\in\LL^*$ and~$\LL^*\circ\LL \subseteq \LL^*$,
    where $\epsilon$~is the empty word.

\begin{proposition}\label{prop:closure}
Languages recognised by HRAs are closed under union, intersection, concatenation and Kleene star.
\end{proposition}

\begin{proof}
We show concatenation and Kleene star only. For the former, consider HRAs $\AA_i=\langle Q_i,q_{0i},H_{0i},\delta_i,F_i\rangle$, $i=1,2$, and assume wlog that they have common type $(m,n)$. Let $w$ be an enlistment of all names in $H_{02}$ and construct $\AA_i'=\fix{\AA_i}{w}$, for $i=1,2$. Then, the concatenation $\LL(\AA_1)\circ\LL(\AA_2)$ is the language recognised by connecting $\AA_1'$ and $\AA_2'$ serially, that is, the automaton obtained by connecting each final state of $\AA_1'$ to the initial state of $\AA_2'$ with a transition labelled $[m{+}n]$, and with initial/final states those of $\AA_1'/\AA_2'$ respectively.

Finally, given an $(m,n)$-HRA $\AA$ and an enlistment $w$ of its initial names, we construct an automaton $\AA'$ by connecting the final states of $\fix{\AA}{w}$ to its initial state with a transition labelled $[m{+}n]$. We can see that $\LL(\AA')=\LL(\AA)^*$.
\end{proof}


As we shall next see, while universality is undecidable for HRAs,
their emptiness problem can be decided by reduction to coverability for transfer-reset vector addition systems. In combination, these results imply that HRAs cannot be effectively complemented. In fact, there are HRA-languages whose complements are not recognisable by HRAs. This can be shown via the following example, adapted from~\cite{Manuel_Ramanujam:2011}.


\begin{lemma}\label{lem:noncomplement}
HRAs are not closed under complementation.
\end{lemma}


\begin{example}\label{ex:complement}
Consider \ %the language
%\begin{align*}
$\LL_4 = \{w\in\names^*\ |\ \text{ not all names of $w$ occur exactly twice in it }\}$,
%\overline{\LL_4} &= \{w\in\names^*\ |\ \text{ all names in $w$ occur exactly twice in it }\}
%\end{align*}
which is accepted by the $(2,0)$-HRA below.
%, where ``$-$" can be any of $\empti,1,2$.%\vspace{-1.5mm}
\begin{center}
\begin{tikzpicture}[automaton]
\node[state,initial] (q0) {$q_0$};
\node[state,accepting] (q1) [right=of q0] {$q_1$};
\node[state] (q2) [right=of q1] {$q_2$};
\node[state,accepting] (q3) [right=of q2] {$q_3$};
\def\loops{
  edge[loop above] node{$\scriptstyle \empti\ta1\,/\,1\ta 1$} ()
%  edge[loop below] node{$\scriptstyle\empti\ta1$} ()
}
\path[transition]
  (q0) \loops edge node[above]{$\scriptstyle\empti\ta2$} (q1)
  (q1) \loops edge node[above]{$\scriptstyle2\ta2$} (q2)
  (q2) \loops edge node[above]{$\scriptstyle2\ta1$} (q3)
  (q3) \loops;
\end{tikzpicture}%\vspace{-1.5mm}
\end{center}
The automaton non-deterministically selects an input name which either appears only once in the input or at least three times.
%
We claim that $\overline{\LL_4}$, the language of all words whose names occur exactly twice in them, is not HRA-recognisable. 
\end{example}

\begin{proof}
Suppose it were recognisable (wlog, \autoref{prop:regs_his}) by an $(m,0)$-HRA $\AA$ with $k$ states. Then, $\AA$ would accept the word
%\[
$w = a_1\ldots a_{k}\,a_1\ldots a_{k}$
%\]
where all $a_i$'s are distinct and do not appear in the initial assignment of $\AA$. 
Let $p=p_1p_2$ be the path in $\AA$ through which $w$ is accepted, with each $p_i$ corresponding to one of the two halves of $w$. Since all $a_i$s are fresh for $\AA$, the non-reset transitions of $p_1$ must carry labels of the form $(\empti,X)$, for some sets $X$.
Let $q$ be a state appearing twice in $p_1$, say $p_1=p_{11}(q)p_{12}(q)p_{13}$. 
Consider now the path $p'=p_1'p_2$ where $p_1'$ is the extension of $p_1$ which repeats $p_{12}$, that is, $p_1'=p_{11}(q)p_{12}(q)p_{12}(q)p_{13}$. We claim that $p'$ is an accepting path in $\AA$. Indeed, by our previous observation on the labels of $p_1$, the path $p_1'$ does not block, i.e.~it cannot reach a transition $q_1\xrightarrow{X\ta Y}q_2$, with $X\not=\empti$, in some configuration $(q_1,H_1)$ such that $H_1\at X=\empti$. 
We need to show that $p_2$ does not block either (in $p'$).
Let us denote $(q,H_1)$ and $(q,H_2)$ the configurations in each of the two visits of $q$ in the run of $p$ on $w$; and let us write $(q,H_3)$ for the third visit in the run of $p_1'$, given that for the other two visits we assume the same configurations as in $p$. Now observe that, for each nonempty $X\subseteq[m]$, repeating $p_{12}$ cannot reduce the number of names appearing precisely in $X$, therefore $|H_2\at X|\leq|H_3\at X|$. The latter implies that, since $p$ does not block, $p'$ does not block either. Now observe that any word accepted by $w'$ is not in $\overline{\LL_4}$, as $p_1'$ accepts more than $k$ distinct names, a contradiction.
\end{proof}

\cutout{
visited twice by $\AA$ while accepting the first half of $w$, and suppose that these visits partition $w$ in $w=uvv'$, where $|u|\geq k$, so that $\AA$ is in configuration $(q,H)$ right after $u$, and in configuration $(q,H')$ right after $uv$. %(we omit register assignments for brevity). 
Then, $w$ is accepted by a run which traverses a path of the form
\begin{equation}\label{eq:path}
q_0\rightarrow\cdots\rightarrow \underbrace{q\rightarrow\cdots\rightarrow q}_p\!\!\!\!\overbrace{\,\,\,\,\rightarrow\cdots\rightarrow q_F}^{p'}
\end{equation}
for some final state $q_F$. The subpath $p'$ cannot be traversed by $\AA$ from configuration $(q,H)$ as then $\AA$ would accept some word $uv''$ of length $<2k$, which cannot be a member of $\overline{\LL_5}$. The only way in which such a traversal can fail is by reaching a transition $q_1'\xrightarrow{X\ta Y}q_2'$ in $p'$ with configuration $(q_1',H_1')$ such that $\bigcap_{i\in X}H_1'(i)=\empti$. On the other hand, in the original run which accepts $w$, this transition is reached with some configuration $(q_1',H_1)$ such that $\bigcap_{i\in X}H_1(i)\not=\empti$. This implies that there is a transition $q_1\xrightarrow{Z\ta X}q_2$ in $p$ such that no clearance of any history in $X$ occurs between $q_2$ and $q_1'$ in~\eqref{eq:path}. We can therefore rewrite~\eqref{eq:path} as \
$
q_0\to\cdots\to q\to\cdots\to q_1\xrightarrow{Z\ta X}q_2\to\cdots\to q\to\cdots\to q_1'\xrightarrow{X\ta Y}q_2'\to\cdots\to q_F
$
and partition $w$ in $w=u_1b_1u_2b_2u_3$ where $b_1,b_2$ the names accepted by the two denoted transitions respectively. Since $|u_1|\geq k$, $b_1$ does not occur in $u_2b_2u_3$. Hence,~\eqref{eq:path} can be traversed in the same way as in the run that accepts $w$ but with the two denoted transitions accepting the same name. That is, the word $u_1b_1u_2b_1u_3$ is also accepted by $\AA$, contradicting $\LL(\AA)=\overline{\LL_3}$.}





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "jour"
%%% End: 

